On the Shapley-like Payoff Mechanisms in Peer-Assisted Services with Multiple Content Providers

This paper studies an incentive structure for cooperation and its stability in peer-assisted services when there exist multiple content providers, using a coalition game theoretic approach. We first consider a generalized coalition structure consisting of multiple providers with many assisting peers, where peers assist providers to reduce the operational cost in content distribution. To distribute the profit from cost reduction to players (i.e., providers and peers), we then establish a generalized formula for individual payoffs when a "Shapley-like" payoff mechanism is adopted. We show that the grand coalition is unstable, even when the operational cost functions are concave, which is in sharp contrast to the recently studied case of a single provider where the grand coalition is stable. We also show that irrespective of stability of the grand coalition, there always exist coalition structures which are not convergent to the grand coalition. Our results give us an important insight that a provider does not tend to cooperate with other providers in peer-assisted services, and be separated from them. To further study the case of the separated providers, three examples are presented; (i) underpaid peers, (ii) service monopoly, and (iii) oscillatory coalition structure. Our study opens many new questions such as realistic and efficient incentive structures and the tradeoffs between fairness and individual providers' competition in peer-assisted services.

==> gnccr_conclusion.tex <==
\section{Concluding Remarks}\label{sec:conc}

% Not yet

A quote from an interview of BBC iPlayer with CNET UK \cite{refiPlayer}:
``{\em Some people didn't like their upload bandwidth being used. It was
  clearly a concern for us, and we want to make sure that everyone is
  happy, unequivocally, using iPlayer.}''

In this paper, we have studied whether the Shapley incentive structure
in peer-assisted services would be in conflict with the pursuit of
profits by rational content providers and peers. A
lesson from our analysis is summarized as: even
though it is righteous to pay peers more because they become relatively
more useful as the number of peer-assisted services increases, the
content providers will not admit that peers should receive
their due deserts. The providers tend to persist in
single-provider coalitions. In the sense of the classical stability
notion, called `core', the cooperation would have been broken even if we
had begun with the grand coalition as the initial condition. Secondly, we
have illustrated yet another problems when we use the Shapley-like
incentive for the exclusive single-provider coalitions.
These results suggest that the profit-sharing system,
Shapley value, and hence its fairness axioms, are not compatible with
the selfishness of the content providers.

